Exploring Attention Map Reuse for Efficient Transformer Neural Networks

Transformer-based deep neural networks have achieved great success in various sequence applications due to their powerful ability to model long-range dependency. The key module of Transformer is self-attention (SA) which extracts features from the entire sequence regardless of the distance between positions. Although SA helps Transformer performs particularly well on long-range tasks, SA requires quadratic computation and memory complexity with the input sequence length. Recently, attention map reuse, which groups multiple SA layers to share one attention map, has been proposed and achieved significant speedup for speech recognition models. In this paper, we provide a comprehensive study on attention map reuse focusing on its ability to accelerate inference. We compare the method with other SA compression techniques and conduct a breakdown analysis of its advantages for a long sequence. We demonstrate the effectiveness of attention map reuse by measuring the latency on both CPU and GPU platforms.

==> section/pruning.tex <==
% ================================================================================ %
\section{Attention Head Pruning}\label{sec:pruning}
% ================================================================================ %

In this section, we analyze \textbf{attention head pruning} for Transformer-based language modeling~\cite{head-pruning}.
First, we explain the layer-wise attention head pruning algorithm.
Second, we introduce the efficient model architecture for attention head pruning.
Finally, we compare the GPU inference time of the original model and the pruned model.


\subsection{Attention Head Pruning}\label{ssec:head_pruning}

Attention head pruning is a compression technique that removes redundant or less important attention heads in SA submodule~\cite{michel2019sixteen,voita2019analyzing}.
However, it is difficult to determine which head to prune; there is no specific metric for the importance, and uniformly removing a certain ratio of heads for every layer may not be an optimal solution.
Trainable attention head pruning automatically decides which head to be removed, starting from the fully converged state where every attention head exists.
During the pruning process, the model learns to adapt to changed architecture while removing attention heads.
For the pruning, the auxiliary gate parameters $g_i \in \{0, 1\}$ is attached to every attention head.
The gate can be interpreted as a switch because the gate value is multiplied by the output of the attention head.
Formally, Eq.~\eqref{eq:mhsa} can be rewritten as the sum of attention heads:
\begin{equation}
    \text{MHSA}(X) = \sum_{h=1}^{H} \text{SA}_h W_{O_h} + b_O \quad (W_{O_h} \in \mathbb{R}^{d_h\times d}).
\end{equation}
Then, the gate is attached for pruning as below:
\begin{equation}
    \text{MHSA}(X) = \frac{H}{\sum_{h=1}^{H} g_i} \sum_{h=1}^{H} g_i \cdot \text{SA}_h W_{O_h} + b_O .
\end{equation}
The scaling term is multiplied to compensate for the change of feature statistics.
Because the binary gate cannot back-propagate the gradient if the gate value is zero, the BinConcrete function is employed for training gate parameters~\cite{binconcrete,batchshaping}.
To encourage the model to turn off the gate\footnote{Without external pressure, the model will always turn on every gates.}, pruning process exploits additional loss to control the sparsity~\cite{head-pruning}.
The overall loss function is the sum of the original task loss and the sparsity loss:
\begin{equation}
    L_{\text{total}} = L_{\text{LM}} + \lambda L_{\text{sparsity}},
\end{equation}
where the first term tries to preserve the language modeling performance and the second term tries to sparsify the model.
$\lambda$ is a sparsity control coefficient.

After pruning, auxiliary gate parameters are fixed and removed.
If the $h\text{-th}$ attention head is pruned, the corresponding parameters ($W_{Q_h}, W_{K_h}, W_{V_h}, W_{O_h}$) are removed together.
The sparsity ratio of attention heads is defined as the number of pruned heads over the number of total heads before the pruning.
Attention head pruning is a structured pruning algorithm that gains inference speed as the sparsity is high.


\subsection{Pruning Analysis}

Language modeling (LM) is a task to model the likelihood of the given text.
For the input token sequence $S=\{s_1, s_2, ... s_T\}$, the goal of LM is to increase the probability of the sentence $P(S)$.
Because $P(S)$ can be factorized as a product of the probability of each token, LM is usually realized as the autoregressive model that predicts the next token based on the information of previous tokens.
\begin{equation}
    P(S) = P(s_1)P(s_2|s_1) \cdots P(s_T|s_{1:T-1}) = \prod_{i=1}^{T} P(s_i|s_{1:i-1})
\end{equation}
However, it is very difficult to consider the entire history because of the hardware limitation.
DNN-based LM handles this problem by exploiting only a limited length of previous history, for example, 256 or 512 tokens.
In other words, the input length for the LM is fixed for most cases.

All-attention Transformer~\cite{all-attention}, the autoregressive Transformer model, is the baseline for our analysis.
All-attention is different from the vanilla Transformer because there is no FF submodule.
Instead, All-attention equips additional module named persistent memory which is considered as an external source during attention map computation.
Figure~\ref{fig:all_attention} illustrates the architecture of All-attention Transformer layer.
% The hidden dimension of the model is 512 and the number of attention heads is 8.
This architecture is suitable for attention head pruning because almost every computation is equally divided by each attention head.
In other words, the computation savings from the pruning can linearly increase proportionally to the number of pruned attention heads.


\begin{figure*}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{figure/all_attention.png}
    \caption{Illustration of the computation flow of an attention head in All-attention Transformer layer.
    Each layer consists of additional persistent memory that performs as supplementary key and value.
    Instead of the persistent memory, there is no feed-forward submodule in All-attention Transformer.
    }
    % \vspace{-0.3cm}
    \label{fig:all_attention}
\end{figure*}

\begin{figure*}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{figure/lm_analysis.png}
    \caption{Inference time (ms) of Transformer language models after attention head pruning.
    The larger $\lambda$ indicates the higher sparsity and $\lambda=0$ indicates the baseline model.
    $x$-axis is the number of tokens in the input sequence.
    }
    % \vspace{-0.3cm}
    \label{fig:pruning_speedup}
\end{figure*}

We apply the attention head pruning procedure explained in Section~\ref{ssec:head_pruning} and evaluate the pruned model.
Table~\ref{tab:pruning_result} shows the number of pruned heads after pruning using different sparsity coefficients $\lambda$.
Although we cannot directly control the sparsity, more attention heads are pruned as $\lambda$ increases.
We can observe that the sparsity is different over layers, and as sparsity increases, the sparsity of each layer becomes more uniform.
We believe that there exist a minimum of necessary attention heads that cannot be removed without hurting the performance.
\setlength{\tabcolsep}{6pt}
\begin{table*}[h]
  \centering
  \vspace{-0.3cm}
  \caption{Number of pruned attention heads per layer.
  Overall, 16 layers $\times 8 = 128$ heads exist in the baseline.
  A layer with a smaller index is closer to the input.}
  \resizebox{1.0\linewidth}{!}{
  \begin{tabular}{c|cccc cccc cccc cccc|c}
    \toprule
    % \diagbox{$\lambda$}{layer}& 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 & 16 & Total & Sparsity (\%) \\
    $\lambda$ & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 & 16 & Sparsity \\
    \midrule
    0.01   & 0 & 5 & 1 & 2 & 2 & 2 & 2 & 1 & 2 & 1 & 0 & 0 & 1 & 0 & 1 & 2 & 17.2 \\
    0.015  & 2 & 4 & 2 & 3 & 4 & 3 & 3 & 2 & 3 & 2 & 1 & 3 & 2 & 2 & 2 & 3 & 32.0 \\
    0.02   & 3 & 6 & 3 & 4 & 5 & 4 & 4 & 4 & 4 & 4 & 4 & 4 & 5 & 5 & 5 & 5 & 53.9 \\
    \bottomrule
    \end{tabular}}
  \label{tab:pruning_result}
%   \vspace{-0.3cm}
\end{table*}
\setlength{\tabcolsep}{4pt}

To evaluate the pruning effect on the GPU inference time, we show the latency of pruned models for different sequence lengths.
Figure~\ref{fig:pruning_speedup} presents the observed latency on a single RTX-Titan GPU.
We can observe that the ratio between four models are consistent through lengths, following the sparsity ratio in Table~\ref{tab:pruning_result}.
The latency of the most sparse model ($\lambda=0.2$) shows almost half time cost compared to the baseline ($\lambda=0$).
For example, the latter processes a sequence length of 384 in 20ms while the former processes a sequence length of 640 in 20ms.

The pruning degrades the language modeling performance, but the loss is in an acceptable range.
The highest sparsity case increases the perplexity from 23.2 to 24.8 (lower is better) using the same input length as the baseline model.
Note that the perplexity can be interpreted as the number of choices the model should select; an increase of 1.6 points of perplexity can be a considerable trade-off depending on the required level of performance.
Furthermore, we mention that the pruned model can utilize longer sequence with a similar latency budget, therefore it can be expected that the gap may be reduced when the pruned model is additionally fine-tuned with longer inputs.


